DataDream: Few-shot Guided Dataset Generation

While text-to-image diffusion models have been shown to achieve state-of-the-art results in image synthesis, they have yet to prove their effectiveness in downstream applications. Previous work has proposed to generate data for image classifier training given limited real data access. However, these methods struggle to generate in-distribution images or depict fine-grained features, thereby hindering the generalization of classification models trained on synthetic datasets. We propose DataDream, a framework for synthesizing classification datasets that more faithfully represents the real data distribution when guided by few-shot examples of the target classes. DataDream fine-tunes LoRA weights for the image generation model on the few real images before generating the training data using the adapted model. We then fine-tune LoRA weights for CLIP using the synthetic data to improve downstream image classification over previous approaches on a large variety of datasets. We demonstrate the efficacy of DataDream through extensive experiments, surpassing state-of-the-art classification accuracy with few-shot data across 7 out of 10 datasets, while being competitive on the other 3. Additionally, we provide insights into the impact of various factors, such as the number of real-shot and generated images as well as the fine-tuning compute on model performance. The code is available at https://github.com/ExplainableML/DataDream.

==> exploration.tex <==





\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccc}
% 
\multicolumn{9}{l}{In every case, accuracies of ResNet50 training from scratch are below 10\%.} \\
% 
\toprule
\multicolumn{3}{l}{\tabletextmultirow{\bf Aircraft dataset, 100 imgs/cls\\ \textbf{CLIP} (fine-tuning with LoRA)}{l}} & \multicolumn{6}{c}{Number of shots} \\ \hline
Data type & Data generation method & Prompt & 0 & 1 & 2 & 4 & 8 & 16 \\
\hline
Real (paper) & - &  
& - & $\mathtt{\sim}$27 & - & - & - & 62.1 \\
Real (Re-run) & - &  
& 24.3 & 27.0 & - & - & - & 62.2  \\
\hline
Synth & zero-shot & \texttt{\{c\} = "[c]"}
& 23.5 &  &  &  &  & \\
Synth & zero-shot & (add more baselines...) 
& ???? &  &  &  &  & \\
\hline
Synth & few-shot & (add more baselines...) 
&  & ? & ? & ? & ? & ? \\
Synth & few-shot (random seed, Textual-inv.)  & \texttt{\{c\} = "<c>"}
&  & 25.2 & - & - & - & 27.9 \\
Synth & few-shot (random seed, Textual-inv.) & \texttt{\{c\} = "<c>, [c]"}
&  & 25.6 & - & - & - & 32.7 \\
Synth & few-shot (best seed, Textual-inv.)  & \texttt{\{c\} = "<c>"}
&  & 22.2 & - & - & - & 32.0 \\
Synth & few-shot (best seed, Textual-inv.) & \texttt{\{c\} = "<c>, [c]"}
&  & 25.5 & - & - & - & 31.7 \\
Synth & few-shot (random seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 44.60 \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & 28.9 & 29.9 & 30.5 & 38.1 & 41.0 \\
Synth & few-shot (best seed, DreamBooth, scale=0.75)  & \texttt{\{c\} = "[c]"}
&  & - & 30.9 & 32.1 & 39.1 & 40.8 \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & 29.9 & 31.7 & 35.8 & 37.7 \\
Synth & few-shot (best seed, DreamBooth, scale=0.25)  & \texttt{\{c\} = "[c]"}
&  & - & 26.9 & 29.1 & 30.0 & 31.2 \\
Synth & few-shot (best seed, DreamBooth, scale=1.1) Extrapolate & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 41.2 \\
Synth & few-shot (best seed, DreamBooth, scale=1.25) Extrapolate & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 39.2 \\
Synth & few-shot (best seed, WaffleDream-Char, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & 27.5 & - & - & - & 42.8 \\
Synth & few-shot (best seed, WaffleDream-Word, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & 27.3 & - & - & - & 41.6 \\
Synth & few-shot (best seed, DreamTextInv-DatasetWise, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & 27.3 & - & - & - & 45.1 \\
\hline
\bf 200 imgs/cls\\
Synth & few-shot (random seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 47.90 \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 44.1 \\
Synth & few-shot (best seed, DreamBooth, scale=0.75)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 44.7 \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 40.2 \\
Synth & few-shot (best seed, DreamBooth, scale=0.25)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 31.4 \\
\hline
\bf 300 imgs/cls\\
Synth & few-shot (random seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 49.84 \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 46.3 \\
Synth & few-shot (best seed, DreamBooth, scale=0.75)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 46.0 \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 42.5 \\
Synth & few-shot (best seed, DreamBooth, scale=0.25)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 32.2 \\
\hline
\bf 400 imgs/cls\\
Synth & few-shot (random seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 50.52 \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 47.0 \\
Synth & few-shot (best seed, DreamBooth, scale=0.75)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 47.5 \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 43.8 \\
Synth & few-shot (best seed, DreamBooth, scale=0.25)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 33.0 \\
\hline
\bf 500 imgs/cls\\
Synth & few-shot (random seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 53.15 \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 48.0 \\
Synth & few-shot (best seed, DreamBooth, scale=0.75)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 48.5 \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 44.2 \\
Synth & few-shot (best seed, DreamBooth, scale=0.25)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & 34.3 \\
\bottomrule
\end{tabular}
}
\vspace{5pt}
\caption{Default template for the prompt is "a photo of a \{c\}". \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name. 
% Data weighting: $\lambda_1 * L_{real} + (1-\lambda_1) * L_{synth}$
}
\vspace{-10pt}
\label{table:main}
\end{table*}






\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llcccccccccc|c}
% 
\toprule
\bf 16-shot & Data Type & ImageNet & Caltech101 & DTD & EuroSAT & FGVC Aircraft & Oxford Pets & Stanford Cars & SUN397 & Food 101 & Flowers 102 & Avg \\ \hline
VPT [ref] & Real & & & 66.1 & & 36.2 & & 69.0 & & & & \\
TPT [ref] & Real & & & 70.7 & & 45.5 & & 81.4 & & & & \\
VPT + TPT [ref] & Real & & & 72.0 & & 48.0 & & 82.0 & & & & \\
LoRA [ref] & Real & & & 74.3 & & 62.09 & & 88.17 & & & & \\
IsSynth [ref] & Real + Synth & & & 73.6 & & 46.7 & & 82.6 & & & & \\
DISEF \cite{dacosta2023diversified} & Real + Synth & & & 75.4 & & 63.89 & & 88.63 & & & & \\ \hline
Ours & Real + Synth & & & \bf 76.3 & & \bf 65.1 & & \bf 90.0 & & & & \\
% WaffleDream (ours) & Real + Synth & & &  & &  & & & & & & \\
\bottomrule
\end{tabular}
}
\vspace{5pt}
\caption{
}
\vspace{-10pt}
\label{table:main}
\end{table*}





\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccc}
% 
\multicolumn{9}{l}{In every case, accuracies of ResNet50 training from scratch are below 10\%.} \\
% 
\toprule
\multicolumn{3}{l}{\tabletextmultirow{\bf Cars, 100 imgs/cls\\ \textbf{CLIP} (fine-tuning with LoRA)}{l}} & \multicolumn{6}{c}{Number of shots} \\ \hline
Data type & Data generation method & Prompt & 0 & 1 & 2 & 4 & 8 & 16 \\
\hline
Real (paper) & - &  
& - & - & - & - & - & 88.2 \\
Real (Re-run) & - &  
& 62.9 & 69.8 & - & - & - & 86.0  \\
\hline
Synth & zero-shot & \texttt{\{c\} = "[c]"}
& 71.1 &  &  &  &  & \\
Synth & zero-shot & (add more baselines...) 
& ???? &  &  &  &  & \\
\hline
Synth & few-shot & (add more baselines...) 
&  & ? & ? & ? & ? & ? \\
% Synth & few-shot (Ours) & \texttt{\{c\} = "<c>"}
% &  & - & - & - & - & - \\
% Synth & few-shot (Ours) & \texttt{\{c\} = "<c>, [c]"}
% &  & 70.2 & - & - & - & 78.9 \\
Synth & few-shot (random seed, Textual-inv.)  & \texttt{\{c\} = "<c>"}
&  & - & - & - & - & - \\
Synth & few-shot (random seed, Textual-inv.) & \texttt{\{c\} = "<c>, [c]"}
&  & 70.2 & - & - & - & 78.9 \\
Synth & few-shot (best seed, Textual-inv.)  & \texttt{\{c\} = "<c>"}
&  & - & - & - & - & - \\
Synth & few-shot (best seed, Textual-inv.) & \texttt{\{c\} = "<c>, [c]"}
&  & - & - & - & - & - \\
Synth & few-shot (best seed, DreamBooth, scale=1.0)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & - \\
Synth & few-shot (best seed, DreamBooth, scale=0.5)  & \texttt{\{c\} = "[c]"}
&  & - & - & - & - & - \\
% \hline
% Synth + Real (paper) & few-shot & baseline: Arxiv2312
% &  & - & - & - & - & 88.6 \\
% Synth + Real (paper) & few-shot & (add more baselines...) 
% &  & ? & ? & ? & ? & ? \\
% Synth + Real & few-shot, weight $\lambda_1=0.2$ (Ours) & \texttt{\{c\} = "<c>"}
% &  & - & - & - & - & 87.3 \\
% Synth + Real & few-shot, weight $\lambda_1=0.5$ (Ours) & \texttt{\{c\} = "<c>"}
% &  & - & - & - & - & 88.8 \\
% Synth + Real & few-shot, weight $\lambda_1=0.8$ (Ours) & \texttt{\{c\} = "<c>"}
% &  & - & - & - & - & 89.4 \\
% Synth + Real & few-shot, weight $\lambda_1=0.2$ (Ours) & \texttt{\{c\} = "<c>, [c]"}
% &  & - & - & - & - & 88.4 \\
% Synth + Real & few-shot, weight $\lambda_1=0.5$ (Ours) & \texttt{\{c\} = "<c>, [c]"}
% &  & - & - & - & - & 89.8 \\
% Synth + Real & few-shot, weight $\lambda_1=0.8$ (Ours) & \texttt{\{c\} = "<c>, [c]"}
% &  & - & - & - & - & 89.9 \\
\bottomrule
\end{tabular}
}
\vspace{5pt}
\caption{Default template for the prompt is "a photo of a \{c\}". \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name. 
% Data weighting: $\lambda_1 * L_{real} + (1-\lambda_1) * L_{synth}$
}
\vspace{-10pt}
\label{table:main}
\end{table*}




\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llcccccc}
\toprule
\multicolumn{2}{l}{\tabletextmultirow{\bf Previous Literature\\ \bf CLIP-FT Aircraft}{l}} & \multicolumn{6}{c}{Number of shots} \\
Method & Data type & 0 & 1 & 2 & 4 & 8 & 16 \\
\hline
CLIP [ref] & - & 24.81 & - & - & - & - & -\\ 
CoOp [ref] & Real & - & $\sim$18 & $\sim$24 & $\sim$30 & $\sim$38 & 48.0\\ 
LoRA [ref] Real & Real & - & \sim27 & \sim31 & \sim39 & \sim48 & 62.1\\ 
IsSynth [ref] & Real + Synth & 30.78 & $\sim$30 & $\sim$34 & $\sim$36 & $\sim$40 & 46.7\\ 
DISEF \cite{dacosta2023diversified} & Real + Synth & - & \sim30 & \sim34 & \sim40 & \sim50 & 63.9\\ \hline
Dreambooth (best seed, scale=1.0) & Real + Synth & - & - & - & - & - & 61.6 \\
Dreambooth (best seed, scale=0.75) & Real + Synth & - & - & - & - & - & 61.6\\
Dreambooth (random seed0, scale=1.0) & Real + Synth & - & - & - & - & - & 65.1\\
\bottomrule
\multicolumn{2}{l}{\tabletextmultirow{\bf CLIP-FT Cars\\ }{l}} & \multicolumn{6}{c}{Number of shots} \\
Method & Data type & 0 & 1 & 2 & 4 & 8 & 16 \\
\hline
CLIP [ref] & - & 65.2 & - & - & - & - & -\\ 
CoOp [ref] & Real & - & - & - & - & - & 81.4\\ 
LoRA [ref] & Real & - & - & - & - & - & 88.2\\ 
IsSynth [ref] & Real + Synth & 66.86 & - & - & - & - & 82.6\\  
DISEF \cite{dacosta2023diversified} & Real + Synth & - & - & - & - & - & 88.6\\ 
\hline
Dreambooth (best seed, scale=1.0) & Real + Synth & - & 62.0 & - & - & - & 89.1\\
Dreambooth (best seed, scale=0.75) & Real + Synth & - & 70.0 & - & - & - & 90.0\\
Dreambooth (random seed0, scale=1.0) & Real + Synth & - & - & - & - & - & 90.0\\
\bottomrule
% 
\end{tabular}
}
\vspace{5pt}
\caption{}
\vspace{-10pt}
\label{table:fid_mmd}
\end{table*}





\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccccc}
% 
\toprule
% \multirow{2}{*}{CLIP}
\multicolumn{2}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \textbf{ResNet50} (training from scratch)}{l}} & \multicolumn{9}{c}{Number of shots} \\ \hline
Data type & Data generation method & 0 & 1 & 2 & 4 & 8 & 16 & 32 & 64 & 500 \\
\hline
% Real (full) & - 
% &  &  &  &  &  &  &  &  & 81.4 \\
% & \multicolumn{5}{c}{-------------- 81.4 --------------} \\
Real & -  
& 0.0 & - & - & - & - & 13.4 & - & - & 81.4 \\
\hline
Synth & zero-shot (name + templates)  
& 56.5 &  &  &  &  &  &  &  &  \\
% & \multicolumn{5}{c}{-------------- 56.5 --------------} \\
Synth & zero-shot (add more baselines...) 
& ???? &  &  &  &  &  &  &  &  \\
% & \multicolumn{5}{c}{-------------- ???? --------------} \\
\hline
Synth & few-shot (add more baselines...)
&  & ? & ? & ? & ? & ? & ? & ? &  \\
Synth & few-shot (Ours)  
&  & 46.4 & 52.4 & 56.9 & 60.2 & 62.9 & 62.3 & 64.8 &  \\
Synth + Real & few-shot (Ours) 
&  & 45.4 & 52.4 & 57.5 & 61.4 & 65.3 & 67.5 & 72.4 &  \\
\bottomrule
% 
% \toprule
% % \multirow{2}{*}{CLIP}
% \multicolumn{2}{l}{\tabletextmultirow{\bf 500 hyperfeatures/cls\\ \textbf{AggNet} (training from scratch)}{l}} & \multicolumn{5}{c}{Number of shots} \\ \hline
% Data type & Data generation method & 1 & 2 & 4 & 8 & 16 \\
% \hline
% Synth & few-shot (Ours)  
% & - & - & - & - & 66.6 \\
% \bottomrule
% 
\toprule
% \multirow{2}{*}{CLIP}
\multicolumn{2}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \textbf{CLIP} (fine-tuning with LoRA)}{l}} & \multicolumn{9}{c}{Number of shots} \\ \hline
Data type & Data generation method & 0 & 1 & 2 & 4 & 8 & 16 & 32 & 64 & 500 \\
\hline
% Real (full) & - 
% &  &  &  &  &  &  &  &  & 93.9 \\
% Real (zero-shot) &   
% & 87.3 &  &  &  &  &  &  &  &  \\
Real & -  
& 87.3 & 89 & 89.8 & 90.4 & 90.8 & 90.9 & 92.0 & 92.5 & 93.9 \\
\hline
Synth & zero-shot (name + templates)  
& 88.0 &  &  &  &  &  &  &  &  \\
Synth & zero-shot (add more baselines...) 
& ???? &  &  &  &  &  &  &  &  \\
\hline
Synth & few-shot (add more baselines...)
&  & ? & ? & ? & ? & ? & ? & ? &  \\
Synth & few-shot (Ours)  
&  & 88.8 & 88.3 & 89.1 & 89.8 & 89.2 & 89.6 & 89.6 &  \\
Synth + Real & few-shot (Ours) 
&  & 87.8 & 88.6 & 88.3 & 90.8 & 91.1 & 92.0 & 92.3 &  \\
\bottomrule
% \toprule
% \multicolumn{2}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \textbf{CLIP} (fine-tuning with LoRA)}{l}} & \multicolumn{5}{c}{Number of shots} \\ \hline
% Data type & Data generation method & 1 & 2 & 4 & 8 & 16 \\
% \hline
% Real (full) & -
% & \multicolumn{5}{c}{-------------- 93.9 --------------} \\
% Real (zero-shot) & - 
% & \multicolumn{5}{c}{-------------- 87.8 --------------} \\
% Real (few-shot) & -
% & 89 & 89.8 & 90.4 & 90.8 & 90.9 \\
% \hline
% Synth & zero-shot (name + templates) 
% & \multicolumn{5}{c}{-------------- 88.0 --------------} \\
% Synth & zero-shot (add more baselines...) 
% & \multicolumn{5}{c}{-------------- ???? --------------} \\
% \hline
% Synth & few-shot (add more baselines...)
% & ? & ? & ? & ? & ? \\
% Synth & few-shot (Ours)
% & 88.8 & 88.3 & 89.1 & 89.8 & 89.2 \\
% Synth + Real & few-shot (Ours)
% & 87.8 & 88.6 & 88.3 & 90.8 & 91.1 \\
% \bottomrule
% 
\end{tabular}
}
\vspace{5pt}
\caption{Ours: the prompt for few-shot guided data generation is \texttt{"a photo of a <c> [c]."} where \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name. }
\vspace{-10pt}
\label{table:main}
\end{table*}



% \clearpage

\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llccccccc}
\toprule
\multicolumn{2}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \textbf{Data Weighting} ($\lambda_1 * L_{real} + (1-\lambda_1) * L_{synth}$)}{l}} & \multicolumn{6}{c}{$\lambda_1$} \\
\hline
Model & Data generation method & 0 & 0.2 & 0.4 & 0.6 & 0.8 & 1 \\
\hline
ResNet50 & 16-shot
& 62.9 & \bf 66.2 & 64.8 & 64.6 & 62.6 & 13.4 \\
CLIP & 16-shot 
& 89.2 & 90.6 & 91.0 & 91.3 & \bf 91.3 & 90.9 \\
\bottomrule
% 
\end{tabular}
}
\vspace{5pt}
\caption{Ours: the prompt for few-shot guided data generation is \texttt{"a photo of a <c> [c]."} where \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name.}
\vspace{-10pt}
\label{table:main2}
\end{table*}


\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llllccccccc}
\toprule
\multicolumn{4}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \textbf{Prompt Weighting} ($w_1 * Emb_{1} + (1-w_1) * Emb_{2}$)}{l}} & \multicolumn{6}{c}{$w_1$} \\
\hline
Model & Data gen. method & Prompt for $Emb_1$ & Prompt for $Emb_2$ & 0 & 0.2 & 0.4 & 0.6 & 0.8 & 1 \\
\hline
ResNet50 & 16-shot, $\lambda_1 = 0.2$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>"} \qquad\qquad\qquad
& - & 64.6 & 60.5 & 59.5 & \bf 64.0 & 56.5 \\
ResNet50 & 16-shot, $\lambda_1 = 0.2$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>, [c]"}
& \bf 66.2 & 61.9 & - & - & 62.4 & 56.5 \\
ResNet50 & 1-shot, $\lambda_1 = 0.2$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>, [c]"}
& 45.4 & 55.0 & - & - & - & \bf 56.5 \\
CLIP & 16-shot, $\lambda_1 = 0.8$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>"}
& - & 91.1 & 91.4 & \bf 91.6 & 91.3 & 88.0 \\
CLIP & 16-shot, $\lambda_1 = 0.8$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>, [c]"}
& 91.3 & 91.4 & - & - & \bf 91.5 & 88.0 \\
CLIP & 1-shot, $\lambda_1 = 0.8$ & \texttt{\{c\} = "[c]"} & \texttt{\{c\} = "<c>, [c]"}
& 87.8 & \bf 89.1 & - & - & 88.8 & 88.0 \\
\bottomrule
% 
\end{tabular}
}
\vspace{5pt}
\caption{Default template for the prompt is "a photo of a \{c\}". \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name.}
\vspace{-10pt}
\label{table:main3}
\end{table*}

\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llcccccc}
\toprule
\multicolumn{2}{l}{\tabletextmultirow{\bf 500 imgs/cls\\ \bf FID}{l}} & \multicolumn{6}{c}{Number of shots} \\
\hline
Data type & Data generation method & 0 & 1 & 2 & 4 & 8 & 16 \\
\hline
Synth & zero-shot
& 72.0 \\
Synth & few-shot (ours)
& & 74.2 & 61.3 & 55.0 & 49.1 & 47.8 \\
\bf MMD & \\
\hline
Synth & zero-shot
& 2.8e-4 \\
Synth & few-shot (ours)
& & 3.0e-4 & 2.8e-4 & 2.8e-4 & 2.7e-4 & 2.6e-4 \\
\bottomrule
% 
\end{tabular}
}
\vspace{5pt}
\caption{Ours: the prompt for few-shot guided data generation is \texttt{"a photo of a <c> [c]."} where \texttt{<c>} is a learned token by textual inversion with few-shot and \texttt{[c]} is a class name. }
\vspace{-10pt}
\label{table:fid_mmd}
\end{table*}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=\linewidth]{images/tmp.PNG} 
%     \caption{.}
%     % \label{fig:main}
% \end{figure}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=\linewidth]{images/mmd_graph.png} 
%     \caption{Histogram of the MMDs per-class for different numbers of shots. 0-shot represents the baseline for synthetic images, name-only. All MMDs are measured for 500 images per class generated by SD2.1.}
%     % \label{fig:main}
% \end{figure}



\section{Training compute}


\begin{table*}[]
\centering
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{llcccccc}
% 
\toprule
\bf Aircraft & Data Type & 50ep & 100ep & 200ep & 300ep & 400ep & 500ep \\ \hline
\ourscls & Synth & 
 & 57.75 & 60.38 & 60.11 &  & \\
\oursdset & Synth & 
 & 64.70 & 71.07 & 71.92 &  & \\
\ourscls & Real + Synth & 
 & 66.81 & 67.00 & 66.93 &  & \\
\oursdset & Real + Synth & 
 & 68.17 & 71.98 & 72.48 &  & \\
\bottomrule
% 
\toprule
\bf EuroSAT & Data Type & 50ep & 100ep & 200ep & 300ep & 400ep & 500ep \\ \hline
\ourscls & Synth & 
- & - & 84.89 & 84.50 & 83.79 & 84.29 \\
\oursdset & Synth & 
- & 71.38 & 79.92 & 77.60 & 82.29 & - \\
\ourscls & Real + Synth & 
 & 92.66 & 93.58 & 93.40 & 93.57 & 93.13 \\
\oursdset & Real + Synth & 
- & 93.50 & 93.39 & 93.53 & 94.05 & - \\
\bottomrule
\end{tabular}
}
\vspace{5pt}
\caption{
    \textbf{Accuracy when increasing the training epochs for dataset-tailored diffusion model fine-tuning.} 
    The accuracy consistently increases then saturates at epoch \todo{200}. 
    \jm{move this to Appendix?}
    \todo{Make the plot instead of table?}
}
\label{tbl:datadream_training_vary}
\vspace{-10pt}
\end{table*}

